Story of Your Lazy Function's Life: A Bidirectional Demand Semantics for Mechanized Cost Analysis of Lazy Programs

Lazy evaluation is a powerful tool that enables better compositionality and potentially better performance in functional programming, but it is challenging to analyze its computation cost. Existing works either require manually annotating sharing, or rely on separation logic to reason about heaps of mutable cells. In this paper, we propose a bidirectional demand semantics that allows for extrinsic reasoning about the computation cost of lazy programs without relying on special program logics. To show the effectiveness of our approach, we apply the demand semantics to a variety of case studies including insertion sort, selection sort, Okasaki's banker's queue, and the implicit queue. We formally prove that the banker's queue and the implicit queue are both amortized and persistent using the Rocq Prover (formerly known as Coq). We also propose the reverse physicist's method, a novel variant of the classical physicist's method, which enables mechanized, modular and compositional reasoning about amortization and persistence with the demand semantics.

==> comparison.tex <==
\section{Comparing the Unknowable Future and the Written Past}\label{sec:comparison}

Relate to clairvoyant semantics

Some relation

\begin{lstlisting}
(a -> M b)   ->   (a0 -> b -> Tick a)   ->    Prop
\end{lstlisting}

\paragraph{The Clairvyant Semantics}

\lx{This could be turned into a comparison between clairvoyant evaluation and
demand functions for reasoning about cost.}

A challenge for formalizing lazy evaluation is that lazy evaluation is
fundamentally stateful, which requires modeling higher-order
stacks~\citep{launchbury1993}, \etc\@ The work of \citet{clairvoyant} and
\citet{forking-paths} work around this challenge by making use of an
``equivalent''\footnote{To be precise, the clairvoyant semantics is only
  equivalent to the natural semantics in terms of pure functional correctness as
  well as computation costs. They are not equivalent, for example, on memory
  usage, \etc} semantics, namely the \emph{clairvoyant semantics}, that uses
\emph{nondeterminism} to simulate laziness. The key idea is to conjecture a
different demand on every nondeterministic branch, so that eventually one of
these branches represent the correct computation cost of a lazy evaluation.

\ly{TODO: explain clairvoyant semantics in more detail. Maybe with a running
  example.}

The issue with the clairvoyant semantics is that we need to ``reduce'' all the
potential nondeterministic results to get an accurate computation cost.
\Citet{clairvoyant} assume that they have the entire program, so that they can
``reduce'' all the nondeterministic results using least fixed points and the
join operation on a lattice. \Citet{forking-paths} look for a modular approach
that only assumes that they have a function. To specify a function in the
presence of nondeterminism, they use two different specifications, a
\emph{\pessim{} specification} that is based on an \emph{over}-approximation,
and an \emph{\optim{} specification} that is based on an
\emph{under}-approximation, similar to the style of incorrectness
logic~\citep{incorrectness, rev-hoare}.

\ly{TODO: an example of dual specification based on the running example.}

However, the \optim{} specification suffers with a compositionality issue. In
the work of \citet{forking-paths}, they insert a \cdc{thunk} combinator to every
function call. The \cdc{thunk} combinator forks the computation into two
nondeterministic branches: on one branch, the function call happens; on the
other branch, the function call is skipped. To reason about the \cdc{thunk}
combinator using the \optim{} specification, one needs to rely one of the
following two rules:\footnote{In the original work by
  \citeauthor{forking-paths}, these two rules are combined as one rule, with a
  disjunction above the line to represent the two
  possibilities~\citep[Fig.~14]{forking-paths}.}
\begin{mathpar}
\inferrule
  {\optimr{u}{\lambda x. r\ (\texttt{Thunk x})}}
  {\optimr{(\texttt{thunk}\ u)}{r}}
  {\hbox{\texttt{thunk}-go}}

\inferrule
  {r\ \texttt{Undefined}\ 0}
  {\optimr{(\texttt{thunk}\ u)}{r}}
  {\hbox{\texttt{thunk}-skip}}
\end{mathpar}
\ly{TODO: explain all the notations and the type of $r$.} We use the first rule,
\ie~\texttt{thunk}-go, when the function call happens. The second rule,
\ie~\texttt{thunk}-skip, is used when the function call is skipped. It usually
requires some manual analysis to decicde which rule to use.

\paragraph{A backward demand semantics}

In this work, we try to address this problem caused by nondeterminism. Our key
idea is: what happens now is \emph{determined if we look back from the future}.
Even though there are multiple possible results given a specific input demand,
there is \emph{only one minimal} input demand given one output
demand.\footnote{As long as nondeterminism is not present in the original
  language.~\ly{We will need to be clear that the ``nondeterminism'' here is for
    the original language; not the nondeterminism we use to simulate laziness.}}
Therefore, instead of using dual specification to specify a clairvoyant
evaluation, we make a ``backward evaluation'' from an output demand to recover
what happens during the clairvoyant evaluation. This is in fact an old idea by
\citet{bjerner1989}---we adapt this idea in this work.\ly{Adapt it to use it in
  clairvoyant semantics? Probably need to compare how different is our work with
  \citet{bjerner1989}.}

Taking \cdc{append [1,2,3] [4]} as an example, if we know that the output demand
is \cdc{[1,2,..]}~(we use \cdc{..} to denote an unevaluated thunk), we know that
the minimal input demands for both arguments must be \cdc{[1,2,..]} and
\cdc{..}, respectively. As a consequence, we are able to know exactly when a
``thunk'' is evaluated or skipped during the evaluation.\ly{TODO: more detail,
  more explanations.}


==> coq.tex <==
\subsection{The Coq Framework}\label{subsec:coq}

In this section, we discuss our Coq framework, which we used to formally
prove that the banker's queue is amortized and persistent.

\paragraph{Approximation datatypes and demand functions}

The first step of formally reasoning about the banker's queue is defining its
approximation datatype (which is also its demand datatype) and its demand
functions. We show the approximation datatype and one example demand function
for the banker's queue in \cref{fig:pushD}.

The banker's queue datatype consists of two natural
numbers and two lists~(\cref{fig:banker-queue}). The approximation datatype of
the banker's queue simply translates all the \cdc{list}s to
\cdc{listA}s.\footnote{We do not have an approximation datatype for \cdc{nat}s.
  This is because, in most programming languages, these numbers will be
  represented using primitive datatypes that do not embed laziness inside their
  structures.} We also define the definedness relations such as
\cdc{less_defined} and \cdc{is_approx} on the queue's approximation datatypes.
We define all these relations using
typeclasses\footnote{\url{https://coq.inria.fr/doc/V8.16.0/refman/addendum/type-classes.html}}
so that they can be overloaded by different data
structures. With \cdc{QueueA}, for instance, we can reuse the relations defined on
\cdc{listA}.

\begin{figure}[t]
\begin{lstlisting}[language=Coq,numbers=left,xleftmargin=4.0ex]
Record QueueA (a : Type) : Type := MkQueueA
  { nfrontA : nat
  ; frontA : T (listA a)
  ; nbackA : nat
  ; backA : T (listA a)
  }.

Definition pushD {a} (q : Queue a) (x : a)
                     (outD : QueueA a) : Tick (T (QueueA a) * T a) :=
  tick >> let+ (frontD, backD) := mkQueueD (nfront q) (front q)
                                   (S (nback q)) (x :: back q) outD in
  ret (Thunk (MkQueueA (nfront q) frontD (nback q) (tailX backD)), Thunk x).
\end{lstlisting}
\caption{Monadic and demand translations of the banker's queue's \cdc{push}
  function.}\label{fig:pushD}
\end{figure}

The demand function \cdc{pushD} is translated manually from
\cdc{push}~(\cref{fig:banker-queue}) by following the demand semantics shown in
\cref{subsec:lazy-semantics}~(\cref{fig:demand-semantics}), but we made some 
simplifications for readability and simplicity. These adjustments
do not impact the correctness of our verification, as we will connect the
queue's demand functions with its clairvoyance semantics when justifying
amortization and persistence.

\paragraph{Cost specification}

Once we have the approximation datatype, demand functions, and the necessary
relations, we can state the cost specification for each demand function and
verify it. We show the cost specification for \cdc{push} in \cref{fig:costspec}.

\begin{figure}
\begin{lstlisting}[language=Coq,numbers=left,xleftmargin=4.0ex]
Definition potential (q: QueueD) : nat :=
  2 * (sizeX 0 (frontD q) - nbackD q).

Definition const : nat := 7.

Theorem push_cost : forall q x qOutD,
  qOutD `is_approx` push q x ->
  let (cost, qInD) := pushD q x qOutD in
  potential qInD + cost <= potential qOutD + const.
\end{lstlisting}
\caption{Cost specification for \cdc{push}.}\label{fig:costspec}
\end{figure}

The cost specification is defined by following the
\method{}~(\cref{sec:physicist}). We define the \potential{}~(lines 1--2) of the
queue to be twice the length of the \emph{demand} of the queue's front list's
minus the length of its back list, as described in
Inequality~\ref{eqn:potential}. The function \cdc{sizeX} measures the ``length''
of a demand list. It is parameterized by a natural number which represents how
long we consider the length of \cdc{NilA} — \ie~\cdc{sizeX 0} means that a demand
list of \cdc{NilA} has a length of \cdc{0}. We then define the cost
specification of \cdc{pushD} as an inequality between the \potential{} of its
input demand~(\cdc{qInD}) plus the cost~(\cdc{cost}) and the \potential{} of its
output demand~(\cdc{qOutD}) plus a constant~(\cdc{const})~(lines 6--9). This is
essentially the same as Inequality~\ref{eqn:costspec} but we change the
inequality to only include the \cdc{+} operation so that we will only need to
use natural numbers in the specification.

\paragraph{Traces}

To show that the banker's queue has amortized constant time cost and that
the queue is persistent, we need to reason about the computation cost of the
queue on \emph{all possible program traces} that use it correctly, \ie~the
trace only uses the queue's ``public'' operations that maintain the queue's
correctness and performance internally. To represent program traces and 
guarantee that values are only ever constructed through the data structure's
interface, our representation of operations (\ie~the \cd{op} type) does not
contain values, but only indirect references to them. \Cref{fig:tracedef}
defines \emph{traces} as sequences of \emph{events}, where each event is a pair
of an operation name (of type \cdc{op}), and a list of pointers (of type
\cdc{nat}) to the result of a past operation. For example, the expression
\cdc{let t = push 42 empty in pop (push 6 t)} is described by the trace
\cdc{[Empty; Push 42 0; Push 6 1; Pop 2]}.

\begin{figure}[t]
\begin{lstlisting}[language=Coq]
(* [op] instantiated by queue operations. *)
Variant op : Type :=
| Empty
| Push (x : a)
| Pop.

(* General definitions of events and traces. *)
Definition event : Type := op * list nat.
Definition trace : Type := list event.
\end{lstlisting}
\caption{Definitions of \cdc{trace} and \cdc{event}.}\label{fig:tracedef}
\end{figure}

% Note that operations may produce zero, one, or many output values, so the
% correspondence between operations and their results may not be
% straightforward. It is not necessary to record it for our purposes.
This approach lets us model the usage of a \emph{persistent data structure}, as
results may be used more than once. A trace encodes a directed acyclic
graph~(DAG) of dependencies between operations. It is a tree if all operations
belonging to the data structure, the first of which takes exactly one input. \lai{Double check that I am understanding this correctly, please!}

\begin{figure}[t]
\begin{lstlisting}[language=Coq]
Definition pushA {a} (q : T (QueueA a)) (x : T a) : M (QueueA a) :=
  tick >>
  let! q := force q in
  mkQueueA (nfrontA q) (frontA q) (S (nbackA q)) (Thunk (ConsA x (backA q))).
\end{lstlisting}
\caption{The clairvoyance function of \cdc{push}.}\label{fig:pushA}
\end{figure}

To ``run'' a trace, we need to define some semantics for all
operations~(\cdc{op}) in a trace. We define three interpreters: a ``pure
interpretation'' \cdc{eval} that interpret each operation using its original
pure definition, a clairvoyant interpretation \cdc{exec} that interprets
operations using the \emph{clairvoyance monad}~\citep{forking-paths}, and a
``budget interpretation'' \cdc{budget} that assigns computation cost budgets to
each operation. The \cdc{eval} interpretation allows us to specify functional
correctness and bound over valid approximations and demands. The \cdc{exec}
interpretation connects our theorems based on demand functions with the trace
based on the clairvoyance monad, which ensures that our proofs show the
correct computation cost of laziness.\footnote{We do not need this extra
  assurance if, \eg~these demand functions are automatically translated using
  the demand semantics shown in \cref{subsec:lazy-semantics}, thanks to
  \cref{thm:fun-correct}--\ref{thm:minimality}.} We show the clairvoyance
function of \cdc{push}~(\cdc{pushA}) in \cref{fig:pushA}. Finally, by
assigning the \cdc{budget} interpretation with a constant number for each
operation, we can show that the banker's queue is both amortized and persistent.

Once we have defined these interpretations for each operation, we can lift them
to the entire trace. \Cref{fig:evaltrace} lifts \cdc{eval}, \cdc{exec}, and
\cdc{budget} to events by composing with an indexing operator \cdc{lookups}, and
to traces by sequencing. \lai{This second sentence is confusing to me (particularly confused what it meant by "sequencing"), but I don't understand the underlying concept well enough to know whether it's my lack of knowledge or something that could be explained more clearly.}
% The definition of \cdc{budget_trace} uses \cdc{eval} since \cdc{budget} must
% be applied to a \cdc{list value}.

\begin{figure}[t]
\codeplus{example.v}{evaltrace}{language=Coq}
\codeplus{example.v}{exectrace}{language=Coq}
\codeplus{example.v}{budgettrace}{language=Coq}
\caption{Sequencing of \cdc{eval}, \cdc{exec}, and \cdc{budget} over
  traces}\label{fig:evaltrace}
\end{figure}

%\begin{figure}[t]
%\codeplus{example.v}{queued}{language=Coq}
%\caption{Translation of the queue to demand functions.}\label{fig:queue-d}
%\end{figure}

\paragraph{Amortization and persistence}

We can show that the banker's queue is amortized and persistent by proving the
following theorem in Coq:
\begin{lstlisting}[language=Coq]
Theorem amortized_cost :
  forall os : trace, (cost_of (exec_trace os) <= budget_trace os).
\end{lstlisting}
This theorem states that for all possible program traces using the banker's
queue, the cost of executing the trace (\ie~running the program) is bounded by a
``budget'' that allocates a constant bound for each operation. Effectively, it states that the banker's
queue has \emph{amortized constant computation cost}. In addition, the theorem
also implies that the banker's queue is \emph{persistent} because the bound is
proven on all traces, including those use the same copy of a queue more than
once.

\iffalse
\paragraph{Uniformly representing operations}

\Cref{fig:opdef} declares a type \cdc{op} of \emph{names} for the operations, a
type \cdc{value} containing the main type(s) of the data structure, and a type
\cdc{valueA} which is the counterpart of \cdc{value} in the monadic translation
in the clairvoyance monad \cdc{M}. For our running example of sequences, we
define \cdc{value} and \cdc{valueA} as the types of sequences of a fixed element
type.

The three sets of functions introduced earlier (pure, monadic, and budget)
can be packed respectively into three functions. Each one takes an operation name
and a list of values to be used as arguments for the corresponding operation,
and outputs a list of values (or a \cdc{nat} for the budget).
\Cref{fig:evaldef} shows the definition of such a function \cdc{eval} from the
pure implementation, and the signatures of the remaining two, \cdc{exec} and
\cdc{budget}. In the cases where the length of the list doesn't match the actual
arity of the operation, we can return the empty list or ignore spurious arguments.

To validate that our cost specification correctly formalizes the idea of
``amortized cost,'' we can show that it lets us bound the cost of whole traces
of execution. This is a generic result: we can prove the correctness of our
``Physicist's method'' for arbitrary data structures. To verify a data structure
using our framework, a user only needs to prove cost specifications of the form
in~\cref{fig:costspec}.

\begin{figure}
\begin{lstlisting}[language=Coq,numbers=left,xleftmargin=4.0ex]
Inductive op : Type :=
| Empty
| Push (x : a)
| Pop.

Definition eval_event : Event Queue -> Queue := ...
Definition eval_trace : Trace -> list Queue := ...

Definition demand_event : Event Queue -> T QueueD -> Tick (T QueueD) := ...
Definition demand_trace : Trace -> list (T QueueD) -> Tick unit := ...
\end{lstlisting}
\caption{Coq definitions related to traces.}\label{fig:traces}
\end{figure}

We show all the Coq definitions related to traces instantiated with the banker's
queue in \cref{fig:traces}. A \cdc{Trace} describes how a data structure is used
in a program: it consists of a sequence of \cdc{Event}s describing operations
made during the execution of the program (line~6). The \cdc{Event} data type has
one constructor for every operation and each constructor is parameterized by the
corresponding operation's inputs (lines~1--4). The \cdc{Event} type is also
parameterized by a state type. In \cref{fig:traces}, the \cdc{Event} type is
instantiated with natural numbers~(\cdc{nat}), which represents the queue's
``version''.\footnote{If the natural number refers to a version of the queue
  that does not exist yet, we can safely ignore the operation.} Given a trace,
we can evaluate it ``forward'' using the pure definitions of the operations
(lines~8--9). We can then evaluate the trace ``backwards'' from a given output
demand (lines~11--12).
% There is no actual input to demand from, so the result is \cdc{Tick unit}, or
% \cdc{nat}.

For example a trace \cdc{[Empty, Push 0 a, Push 1 b, Push 2 c, Push 3 d, Pop 4,
  Pop 5, Pop 4]} represents the evaluation of each binding of the following
program (using Haskell's BangPatterns\ly{Why BangPatterns here?} to force each
binding to WHNF)---note the repetition of Pop 4 which means the intermediate
queue \cdc{q4} gets reused:

In that sense, traces are really DAGs: the output of every operation may be used
by more than one operation. Beyond \cdc{push} and \cdc{pop}, our framework also
supports data structures with operation that have more than one input (e.g.,
\cdc{append} for sequences) or more than one output (e.g., \cdc{splitAt}).

The budget of operations can be defined uniformly as a function from events to
cost. For queues, the budget can be made constant (as the max budget over all operations),
but in general it may depend on the input.

\begin{lstlisting}[language=Coq]
Definition budget : Event Queue -> nat
 := fun _ => 3.
\end{lstlisting}

We can then sum the budget over a trace:

\begin{lstlisting}[language=Coq]
Definition budget_trace : Trace -> nat.
\end{lstlisting}

The final theorem is that the budget bounds the cost semantics \cdc{demand_trace}.

\begin{lstlisting}[language=Coq]
Theorem correct_budget :
  demand_trace t (bottom_of (eval_trace t)) <= budget_trace t.
\end{lstlisting}
\fi

\begin{figure}[t]
\begin{lstlisting}[language=Coq]
Definition AmortizedCostSpec : Prop :=
  forall os : trace, (cost_of (exec_trace os) <= budget_trace os).
\end{lstlisting}
\codeplus{example.v}{physicist}{language=Coq}
\caption{The physicist's method as a theorem}\label{fig:physicist}
\end{figure}

\paragraph{The \method}

It is challenging to prove the \cdc{amortized_cost} theorem directly. Instead of
reasoning over arbitrary traces, we first prove cost specifications for each
individual operation as shown in \cref{fig:costspec}. We then prove that these
cost specifications imply \cdc{amortized_cost} by formally proving the reasoning
behind the \method, as shown in \cref{fig:physicist}. \lai{Do we need to explain the proof a little here, or are we limiting this section to strictly the specification?}



% \subsection{Limitations}\label{subsec:method-limitations}

% \lx{There are omitted side conditions to discuss at some point.}
% 
% The \cdc{Physicist'sArgument} can be seen as a backwards computation: given an
% \cdc{output} parameter approximating the actual output of an operation, we must
% construct an \cdc{input} argument for the operation which is sufficiently
% defined to match the output, but which also has a small enough potential for the
% cost inequality to hold.
% 
% Our solution is to explicitly define this mapping from \emph{output demands} to
% \emph{input demands}. This is obtained by another translation of the implementation
% to \emph{demand functions}, \Cref{fig:pushD}.
% 
% The \cdc{Physicist'sArgument} can then be decomposed in two steps:
% a simulation proof between the monadic and the demand translation
% (which should be a general theorem about the translations),
% and a variant of \cdc{Physicist'sArgument} for demand functions,
% \Cref{fig:physicistD}.
% 
% \begin{figure}
% \codeplus{example.v}{physicistD}{language=Coq}
% \caption{Demand-function variant of \cdc{Physicist'sArgument}}\label{fig:physicistD}
% \end{figure}

